MACARONS: Mapping And Coverage Anticipation with RGB Online Self-Supervision

We introduce a method that simultaneously learns to explore new large environments and to reconstruct them in 3D from color images only. This is closely related to the Next Best View problem (NBV), where one has to identify where to move the camera next to improve the coverage of an unknown scene. However, most of the current NBV methods rely on depth sensors, need 3D supervision and/or do not scale to large scenes. Our method requires only a color camera and no 3D supervision. It simultaneously learns in a self-supervised fashion to predict a "volume occupancy field" from color images and, from this field, to predict the NBV. Thanks to this approach, our method performs well on new scenes as it is not biased towards any training 3D data. We demonstrate this on a recent dataset made of various 3D scenes and show it performs even better than recent methods requiring a depth sensor, which is not a realistic assumption for outdoor scenes captured with a flying drone.

==> figs/trajectories.tex <==
\begin{figure}
  \centering
  \begin{subfigure}{0.46\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{images/trajectories/fushimi_macarons_1.png}
    \caption{Fushimi Castle}
    \label{fig:traj-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.46\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{images/trajectories/liberty2_macarons.png}
    \caption{Statue of Liberty}
    \label{fig:traj-b}
  \end{subfigure}\\
  \begin{subfigure}{0.46\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{images/trajectories/pantheon_2_macarons.png}
    \caption{\scriptsize Pantheon}
    \label{fig:traj-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.46\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{images/trajectories/neus_7.png}
    \caption{\scriptsize Neuschwanstein Castle}
    \label{fig:traj-d}
  \end{subfigure}
  \caption{{\bf Trajectories computed in real-time by MACARONS in large 3D structures.} MACARONS predicts a NBV at each time step $t$ to build trajectories that consistently cover most of the surface of the scene. MACARONS performed 100 NBV iterations in these images.}
  \label{fig:trajectories}
\end{figure}

==> supp_mat/figs/occupancy.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/pisa_occ.png}
    \caption{Pisa Cathedral}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/pisa_rec.png}
    \caption{Pisa Cathedral}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/liberty_occ.png}
    \caption{Statue of Liberty}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/liberty_rec.png}
    \caption{Statue of Liberty}
  \end{subfigure}
  \hfill \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/pantheon_occ.png}
    \caption{Pantheon}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/pantheon_rec.png}
    \caption{Pantheon}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/fushimi_occ.png}
    \caption{Fushimi Castle}
  \end{subfigure} 
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/fushimi_rec.png}
    \caption{Fushimi Castle}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/colosseum_occ.png}
    \caption{Colosseum}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/colosseum_rec.png}
    \caption{Colosseum}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/neus_occ.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/neus_rec.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure}
  \caption{{\bf Volume occupancy fields computed with our approach MACARONS.} Our model updates the volume occupancy field in real time during exploration: For several scene, we show here the volume occupancy after 100 NBV iterations (left), as well as the final reconstructed surface for comparison (right).% The model has been trained on a set of previous scenes; all weights  are frozen and we only perform inference computation. The first four rows depict scenes that were already seen by the model during its online, self-supervised training. The last two rows depicts scenes the model has never seen before.
  }
  \label{fig:supp-mat-occupancy}
\end{figure*}

\begin{comment}
\begin{figure*}
  \centering
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/pisa_occ.png}
    \caption{Pisa Cathedral}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/pisa_rec.png}
    \caption{Pisa Cathedral}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/liberty_occ.png}
    \caption{Statue of Liberty}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/liberty_rec.png}
    \caption{Statue of Liberty}
  \end{subfigure}
  \hfill \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/pantheon_occ.png}
    \caption{Pantheon}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/pantheon_rec.png}
    \caption{Pantheon}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/fushimi_occ.png}
    \caption{Fushimi Castle}
  \end{subfigure} 
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/fushimi_rec.png}
    \caption{Fushimi Castle}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/colosseum_occ.png}
    \caption{Colosseum}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/colosseum_rec.png}
    \caption{Colosseum}
  \end{subfigure}
  \hfill

  \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/dunnottar_occ.png}
    \caption{Dunnottar Castle}
  \end{subfigure}
  \hfill

    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/dunnottar_rec.png}
    \caption{Dunnottar Castle}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/redeemer_occ.png}
    \caption{Christ the Redeemer}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/redeemer_rec.png}
    \caption{Christ the Redeemer}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/bannerman_occ.png}
    \caption{Bannerman Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/bannerman_rec.png}
    \caption{Bannerman Castle}
  \end{subfigure}\\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/alhambra_occ.png}
    \caption{Alhambra Palace}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/alhambra_rec.png}
    \caption{Alhambra Palace}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/neus_occ.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/neus_rec.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure}\\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/eiffel_occ.png}
    \caption{Eiffel Tower}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/eiffel_rec.png}
    \caption{Eiffel Tower}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/bridge_occ.png}
    \caption{Manhattan Bridge}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/images/occupancy/bridge_rec.png}
    \caption{Manhattan Bridge}
  \end{subfigure}
  \caption{{\bf Volume occupancy fields computed with our approach MACARONS.} Our model updates the volume occupancy field in real time during exploration: For several scene, we show here the volume occupancy after 100 NBV iterations (left), as well as the final reconstructed surface for comparison (right).% The model has been trained on a set of previous scenes; all weights  are frozen and we only perform inference computation. The first four rows depict scenes that were already seen by the model during its online, self-supervised training. The last two rows depicts scenes the model has never seen before.
  }
  \label{fig:supp-mat-occupancy}
\end{figure*}
\end{comment}

==> supp_mat/figs/recons.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pisa_1_color.png}
    \caption{Pisa Cathedral}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pisa_1.png}
    \caption{Pisa Cathedral}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/liberty_2_color.png}
    \caption{Statue of Liberty}
  \end{subfigure} 
  \hfill 
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/liberty_2.png}
    \caption{Statue of Liberty}
  \end{subfigure}\\
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pantheon_1_color.png}
    \caption{Pantheon}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pantheon_1.png}
    \caption{Pantheon}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/fushimi_1_color.png}
    \caption{Fushimi Castle}
  \end{subfigure}
  \hfill 
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/fushimi_1.png}
    \caption{Fushimi Castle}
  \end{subfigure}
  \hfill 
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/colosseum_3_color.png}
    \caption{Colosseum}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/colosseum_3.png}
    \caption{Colosseum}
  \end{subfigure} 
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/dunnottar_2_color.png}
    \caption{Dunnottar Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/dunnottar_2.png}
    \caption{Dunnottar Castle}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/redeemer_1_color.png}
    \caption{Christ the Redeemer}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/redeemer_1.png}
    \caption{Christ the Redeemer}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/bannerman_1_color.png}
    \caption{Bannerman Castle}
  \end{subfigure}
  \hfill 
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/bannerman_1.png}
    \caption{Bannerman Castle}
  \end{subfigure}
  \hfill 
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/alhambra_2_color.png}
    \caption{Alhambra Palace}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/alhambra_2.png}
    \caption{Alhambra Palace}
  \end{subfigure} 
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/neusch_2_color.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/neusch_2.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure} 
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/eiffel_2_color.png}
    \caption{Eiffel Tower}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/eiffel_2.png}
    \caption{Eiffel Tower}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=\linewidth]{supp_mat/surface_rec/manhattan_1_color.png}
    \caption{Manhattan Bridge}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=\linewidth]{supp_mat/surface_rec/manhattan_1.png}
    \caption{Manhattan Bridge}
  \end{subfigure}
  \caption{{\bf Automated reconstruction of large 3D structures from RGB images with our approach MACARONS.}   
  Our model reconstructs the surface in real time during exploration: We show here the reconstruction after 100 NBV iterations. The model has been trained on a set of previous scenes; all weights are frozen and we only perform inference computation. The first four rows depict scenes that were already seen by the model during its online, self-supervised training. The two last row depicts scenes the model has never seen before. For each scene, we provide images with colors computed from the input RGB images as well as images for which all points share the same color. The latter help to better estimate the quality of the reconstructed geometry. MACARONS is not only able to reconstruct surfaces thanks to its depth prediction module (even for scenes it has never seen before), but is also able to optimize its path around the structure and consistently cover most of the surface of the scene thanks to its NBV prediction.
  }
  \label{fig:supp-mat-surface-reconstruction-1}
\end{figure*}
%
\begin{comment}
\begin{figure*}
  \centering
  \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pisa_1_color.png}
    \caption{Pisa Cathedral}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pisa_1.png}
    \caption{Pisa Cathedral}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pisa_2_color.png}
    \caption{Pisa Cathedral}
  \end{subfigure}
  \hfill
      \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pisa_2.png}
    \caption{Pisa Cathedral}
  \end{subfigure}\\
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/liberty_1_color.png}
    \caption{Statue of Liberty}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/liberty_1.png}
    \caption{Statue of Liberty}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/liberty_2_color.png}
    \caption{Statue of Liberty}
  \end{subfigure} 
  \hfill 
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/liberty_2.png}
    \caption{Statue of Liberty}
  \end{subfigure}\\
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pantheon_1_color.png}
    \caption{Pantheon}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pantheon_1.png}
    \caption{Pantheon}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pantheon_2_color.png}
    \caption{Pantheon}
  \end{subfigure} 
  \hfill
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/pantheon_2.png}
    \caption{Pantheon}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/fushimi_1_color.png}
    \caption{Fushimi Castle}
  \end{subfigure}
  \hfill 
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/fushimi_1.png}
    \caption{Fushimi Castle}
  \end{subfigure}
  \hfill 
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/fushimi_2_color.png}
    \caption{Fushimi Castle}
  \end{subfigure}
  \hfill 
    \begin{subfigure}{0.23\linewidth}
    % \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/fushimi_2.png}
    \caption{Fushimi Castle}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/colosseum_2_color.png}
    \caption{Colosseum}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/colosseum_2.png}
    \caption{Colosseum}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/colosseum_3_color.png}
    \caption{Colosseum}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/colosseum_3.png}
    \caption{Colosseum}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/dunnottar_1_color.png}
    \caption{Dunnottar Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/dunnottar_1.png}
    \caption{Dunnottar Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/dunnottar_2_color.png}
    \caption{Dunnottar Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/dunnottar_2.png}
    \caption{Dunnottar Castle}
  \end{subfigure} \\
  \caption{{\bf Automated reconstruction of large 3D structures from RGB images with our approach MACARONS.} Our model reconstructs the surface in real time during exploration: We show here the reconstruction after 100 NBV iterations. The model has been trained on a set of previous scenes; all weights  are frozen and we only perform inference computation. In this Figure, all rows depict scenes that were already seen by the model during its online, self-supervised training. For each scene, we provide images with colors computed from the input RGB images as well as images for which all points share the same color. The latter help to better estimate the quality of the reconstructed geometry. MACARONS is not only able to reconstruct surfaces thanks to its depth prediction module, but is also able to optimize its path around the structure and consistently cover most of the surface of the scene thanks to its NBV prediction.}
  \label{fig:supp-mat-surface-reconstruction-1}
\end{figure*}
%
\begin{figure*}
  \centering
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/redeemer_1_color.png}
    \caption{Christ the Redeemer}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/redeemer_1.png}
    \caption{Christ the Redeemer}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/redeemer_2_color.png}
    \caption{Christ the Redeemer}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/redeemer_2.png}
    \caption{Christ the Redeemer}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/bannerman_1_color.png}
    \caption{Bannerman Castle}
  \end{subfigure}
  \hfill 
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/bannerman_1.png}
    \caption{Bannerman Castle}
  \end{subfigure}
  \hfill 
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/bannerman_2_color.png}
    \caption{Bannerman Castle}
  \end{subfigure}
  \hfill 
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/bannerman_2.png}
    \caption{Bannerman Castle}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/alhambra_1_color.png}
    \caption{Alhambra Palace}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/alhambra_1.png}
    \caption{Alhambra Palace}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/alhambra_2_color.png}
    \caption{Alhambra Palace}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/alhambra_2.png}
    \caption{Alhambra Palace}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/neusch_1_color.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/neusch_1.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/neusch_2_color.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/neusch_2.png}
    \caption{Neuschwanstein Castle}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/eiffel_1_color.png}
    \caption{Eiffel Tower}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/eiffel_1.png}
    \caption{Eiffel Tower}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/eiffel_2_color.png}
    \caption{Eiffel Tower}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    \includegraphics[width=\linewidth]{supp_mat/surface_rec/eiffel_2.png}
    \caption{Eiffel Tower}
  \end{subfigure} \\
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=\linewidth]{supp_mat/surface_rec/manhattan_1_color.png}
    \caption{Manhattan Bridge}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=\linewidth]{supp_mat/surface_rec/manhattan_1.png}
    \caption{Manhattan Bridge}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=\linewidth]{supp_mat/surface_rec/manhattan_2_color.png}
    \caption{Manhattan Bridge}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    %\fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=\linewidth]{supp_mat/surface_rec/manhattan_2.png}
    \caption{Manhattan Bridge}
  \end{subfigure} \\
  \caption{{\bf Automated reconstruction of large 3D structures from RGB images with our approach MACARONS.} Our model reconstructs the surface in real time during exploration: We show here the reconstruction after 100 NBV iterations. The model has been trained on a set of previous scenes; all weights  are frozen and we only perform inference computation. The first two rows depict scenes that were already seen by the model during its online, self-supervised training. The four last row depicts scenes the model has never seen before. For each scene, we provide images with colors computed from the input RGB images as well as images for which all points share the same color. The latter help to better estimate the quality of the reconstructed geometry. MACARONS is not only able to reconstruct surfaces thanks to its depth prediction module (even for scenes it has never seen before), but is also able to optimize its path around the structure and consistently cover most of the surface of the scene thanks to its NBV prediction.}
  \label{fig:supp-mat-surface-reconstruction-2}
\end{figure*}

\end{comment}

==> supp_mat/figs/rgb_depth.tex <==
\begin{figure}
  \centering

  \begin{subfigure}{0.23\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    %\includegraphics[width=\linewidth]{images/occupancy_probability/pantheon_t0.png}
    % \caption{Statue of Liberty.}
    %\label{fig:occ-b}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    %\includegraphics[width=\linewidth]{images/occupancy_probability/pantheon_t1.png}
    % \caption{Statue of Liberty.}
    %\label{fig:occ-c}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    %\includegraphics[width=\linewidth]{images/occupancy_probability/pantheon_t2.png}
    % \caption{Statue of Liberty.}
    %\label{fig:occ-d}
  \end{subfigure}
  \hfill
    \begin{subfigure}{0.23\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    %\includegraphics[width=\linewidth]{images/occupancy_probability/pantheon_comparison.png}
    % \caption{Pisa Cathedral.}
    %\label{fig:occ-a}
  \end{subfigure}\\
  \begin{subfigure}{0.23\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    %\includegraphics[width=\linewidth]{images/occupancy_probability/pisa_t0.png}
    \caption{\scriptsize $I_{t-2}$}
    %\label{fig:occ-b-bis}
  \end{subfigure}
    \hfill
  \begin{subfigure}{0.23\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    % \includegraphics[width=\linewidth]{images/occupancy_probability/pisa_t1.png}
    % \caption{Statue of Liberty.}
    \caption{\scriptsize $I_{t-1}$}
    % \label{fig:occ-c-bis}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    % \includegraphics[width=\linewidth]{images/occupancy_probability/pisa_t2.png}
    % \caption{Statue of Liberty.}
    \caption{\scriptsize $I_t$}
    % \label{fig:occ-d-bis}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.23\linewidth}
    \fbox{\rule{0pt}{0.5in} \rule{.9\linewidth}{0pt}}
    % \includegraphics[width=\linewidth]{images/occupancy_probability/pisa_comparison.png}
    \caption{\scriptsize $d_t$}
    % \label{fig:occ-a-bis}
  \end{subfigure}
%   \caption{{\bf Volume occupancy probability field of large 3D structures.} The second module of MACARONS predicts and updates in real-time a volume occupancy probability field (right) from the reconstructed surface points (left).}
  \caption{\textbf{Depth prediction from a sequence of RGB images by our model MACARONS.} At time step $t$, the depth prediction module of MACARONS takes as input the RGB images $I_t, I_{t-1}, ..., I_{t-m}$ to predict the depth map $d_t$. We take $m=2$ in our experiments.}
  \label{fig:supp-mat-rgb-depth}
\end{figure}
